GASKAP-HI Pilot Survey Science III: An unbiased view of cold gas in the Small Magellanic Cloud

We present the first unbiased survey of neutral hydrogen (HI) absorption in the Small Magellanic Cloud (SMC). The survey utilises pilot HI observations with the Australian Square Kilometre Array Pathfinder (ASKAP) telescope as part of the Galactic ASKAP HI (GASKAP-HI) project whose dataset has been processed with the GASKAP-HI absorption pipeline, also described here. This dataset provides absorption spectra towards 229 continuum sources, a 275% increase in the number of continuum sources previously published in the SMC region, as well as an improvement in the quality of absorption spectra over previous surveys of the SMC. Our unbiased view, combined with the closely matched beam size between emission and absorption, reveals a lower cold gas faction (11%) than the 2019 ATCA survey of the SMC and is more representative of the SMC as a whole. We also find that the optical depth varies greatly between the SMC's bar and wing regions. In the bar we find that the optical depth is generally low (correction factor to the optically thin column density assumption of $\mathcal{R}_{\rm HI} \sim 1.04$) but increases linearly with column density. In the wing however, there is a wide scatter in optical depth despite a tighter range of column densities.

==> SMC Absorption With GASKAP-20220410/absorption_table.tex <==
\begin{tabular}{llrrrrrrr}
\hline \hline
Source & Feature & Min Velocity & Max Velocity & Width & Peak & Peak $\tau$ & Significance & Equiv. Width \\
 &  & (kms$^{-1}$) & (kms$^{-1}$) & (kms$^{-1}$) & Absorption &  & (sigma) & (kms$^{-1}$) \\
\hline
J004956$-$723554 & J004956$-$723554\_$-$2 & $-2.3$ & $-0.3$ & 3 & $0.16\pm0.04$ & $0.18\pm0.05$ & 4.1 & $0.45\pm0.07$ \\
J004956$-$723554 & J004956$-$723554\_137 & $137.7$ & $150.7$ & 14 & $0.51\pm0.05$ & $0.72\pm0.10$ & 10.1 & $5.37\pm0.20$ \\
J004956$-$723554 & J004956$-$723554\_155 & $155.7$ & $160.7$ & 6 & $0.45\pm0.05$ & $0.60\pm0.09$ & 8.7 & $2.13\pm0.13$ \\
J004956$-$723554 & J004956$-$723554\_3 & $3.7$ & $4.7$ & 2 & $0.18\pm0.04$ & $0.19\pm0.05$ & 4.6 & $0.38\pm0.06$ \\
J005014$-$730326 & J005014$-$730326\_152 & $152.9$ & $153.9$ & 2 & $1.06\pm0.32$ & $>1.14$ & 3.3 & $2.28\pm0.54$ \\
J005141$-$725545 & J005141$-$725545\_106 & $106.8$ & $108.8$ & 3 & $0.71\pm0.19$ & $1.24\pm0.51$ & 3.8 & $3.18\pm0.37$ \\
J005141$-$725545 & J005141$-$725545\_114 & $114.8$ & $117.8$ & 4 & $1.03\pm0.24$ & $>1.45$ & 4.5 & $6.55\pm0.52$ \\
J005141$-$725603 & J005141$-$725603\_113 & $113.8$ & $120.8$ & 8 & $1.19\pm0.24$ & $>1.44$ & 5.0 & $15.96\pm0.76$ \\
J005218$-$722708 & J005218$-$722708\_0 & $-0.4$ & $1.6$ & 3 & $0.13\pm0.02$ & $0.14\pm0.03$ & 5.8 & $0.31\pm0.04$ \\
J005218$-$722708 & J005218$-$722708\_153 & $153.6$ & $159.6$ & 7 & $0.20\pm0.03$ & $0.22\pm0.04$ & 6.5 & $0.98\pm0.08$ \\
J005218$-$722708 & J005218$-$722708\_161 & $161.6$ & $162.6$ & 2 & $0.12\pm0.03$ & $0.13\pm0.03$ & 4.0 & $0.21\pm0.04$ \\
J005238$-$731245 & J005238$-$731245\_0 & $-0.0$ & $1.0$ & 2 & $0.20\pm0.04$ & $0.22\pm0.05$ & 4.6 & $0.35\pm0.06$ \\
J005238$-$731245 & J005238$-$731245\_132 & $133.0$ & $166.0$ & 34 & $0.96\pm0.06$ & $3.26\pm0.92$ & 16.5 & $35.60\pm0.35$ \\
J005238$-$731245 & J005238$-$731245\_169 & $170.0$ & $174.0$ & 5 & $0.31\pm0.05$ & $0.37\pm0.07$ & 6.2 & $1.47\pm0.12$ \\
J005337$-$723144 & J005337$-$723144\_102 & $102.6$ & $107.6$ & 6 & $0.27\pm0.06$ & $0.31\pm0.07$ & 4.7 & $1.40\pm0.15$ \\
J005337$-$723144 & J005337$-$723144\_122 & $122.6$ & $124.6$ & 3 & $0.35\pm0.08$ & $0.44\pm0.12$ & 4.4 & $1.21\pm0.14$ \\
J005337$-$723144 & J005337$-$723144\_127 & $127.6$ & $134.6$ & 8 & $1.05\pm0.07$ & $>2.61$ & 14.3 & $9.35\pm0.21$ \\
J005423$-$725257 & J005423$-$725257\_122 & $122.8$ & $125.8$ & 4 & $1.18\pm0.19$ & $>1.68$ & 6.3 & $4.87\pm0.41$ \\
J005423$-$725257 & J005423$-$725257\_174 & $174.8$ & $176.8$ & 3 & $0.69\pm0.15$ & $1.17\pm0.38$ & 4.7 & $2.74\pm0.27$ \\
J005448$-$725353 & J005448$-$725353\_116 & $116.8$ & $118.8$ & 3 & $1.12\pm0.31$ & $>1.17$ & 3.6 & $7.67\pm0.63$ \\
J005448$-$725353 & J005448$-$725353\_163 & $163.8$ & $167.8$ & 5 & $1.48\pm0.31$ & $>1.18$ & 4.8 & $11.32\pm0.82$ \\
J005535$-$723533 & J005535$-$723533\_113 & $113.6$ & $114.6$ & 2 & $1.33\pm0.25$ & $>1.38$ & 5.3 & $5.98\pm0.42$ \\
J005535$-$723533 & J005535$-$723533\_116 & $116.6$ & $117.6$ & 2 & $1.07\pm0.27$ & $>1.31$ & 4.0 & $2.83\pm0.45$ \\
J005642$-$725216 & J005642$-$725216\_158 & $158.7$ & $160.7$ & 3 & $1.11\pm0.21$ & $>1.58$ & 5.4 & $5.53\pm0.40$ \\
J005644$-$725200 & J005644$-$725200\_117 & $117.7$ & $118.7$ & 2 & $0.50\pm0.15$ & $0.69\pm0.25$ & 3.4 & $1.30\pm0.22$ \\
J005644$-$725200 & J005644$-$725200\_155 & $155.7$ & $160.7$ & 6 & $1.09\pm0.14$ & $>1.94$ & 7.6 & $6.66\pm0.38$ \\
J005644$-$725200 & J005644$-$725200\_171 & $171.7$ & $172.7$ & 2 & $0.51\pm0.14$ & $0.71\pm0.25$ & 3.7 & $1.32\pm0.21$ \\
J005644$-$725200 & J005644$-$725200\_175 & $175.7$ & $177.7$ & 3 & $0.57\pm0.13$ & $0.84\pm0.26$ & 4.5 & $1.86\pm0.23$ \\
\hline
\end{tabular}


==> SMC Absorption With GASKAP-20220410/spectra_table.tex <==
\begin{tabular}{rcrrrcrrrrr}
\hline \hline
ID & Source & RA & Dec & Peak Flux & Rating & $\sigma_{\rm cont}$ & Peak $\tau$ & N$_{\rm HI,uncorr}$ & $\langle T_{\rm S} \rangle$ & $\mathcal{R}_{\rm HI}$ \\
 &  & (deg) & (deg) & (mJy) &  &  &  & ($10^{21}$ cm$^{-2}$) &  &  \\
\hline
178 & J004718$-$723947 & 11.8285 & $-72.663$ & 32 & B & 0.133 & $0.99\pm0.43$ & 4.0 & $265^{+76}_{-45}$ & $1.10^{+0.02}_{-0.02}$ \\
304 & J004956$-$723554 & 12.4863 & $-72.599$ & 82 & A & 0.034 & $0.72\pm0.10$ & 4.2 & $321^{+26}_{-21}$ & $1.08^{+0.01}_{-0.00}$ \\
33 & J005014$-$730326 & 12.5617 & $-73.057$ & 17 & C & 0.197 & $>1.12$ & 10.3 & $482^{+147}_{-97}$ & $1.23^{+0.04}_{-0.05}$ \\
74 & J005141$-$725545 & 12.9231 & $-72.929$ & 17 & B & 0.136 & $>1.45$ & 8.6 & $260^{+32}_{-26}$ & $1.31^{+0.05}_{-0.04}$ \\
75 & J005141$-$725603 & 12.9216 & $-72.934$ & 19 & B & 0.137 & $>1.44$ & 8.6 & $251^{+35}_{-24}$ & $1.32^{+0.05}_{-0.04}$ \\
62 & J005217$-$730157 & 13.0714 & $-73.033$ & 18 & B & 0.146 & $1.28\pm0.63$ & 7.8 & $291^{+47}_{-39}$ & $1.22^{+0.04}_{-0.04}$ \\
357 & J005218$-$722708 & 13.0779 & $-72.452$ & 153 & B & 0.019 & $0.22\pm0.04$ & 3.9 & $937^{+131}_{-94}$ & $1.02^{+0.00}_{-0.00}$ \\
319 & J005238$-$731245 & 13.1589 & $-73.213$ & 101 & A & 0.035 & $3.26\pm0.92$ & 8.9 & $234^{+7}_{-6}$ & $1.38^{+0.03}_{-0.02}$ \\
287 & J005337$-$723144 & 13.4067 & $-72.529$ & 69 & A & 0.047 & $>2.61$ & 5.0 & $232^{+15}_{-13}$ & $1.12^{+0.02}_{-0.01}$ \\
200 & J005423$-$725257 & 13.5979 & $-72.883$ & 35 & B & 0.105 & $>1.68$ & 7.6 & $405^{+79}_{-53}$ & $1.15^{+0.03}_{-0.02}$ \\
19 & J005448$-$725353 & 13.7026 & $-72.898$ & 16 & C & 0.181 & $>1.18$ & 7.4 & $224^{+40}_{-28}$ & $1.32^{+0.06}_{-0.05}$ \\
13 & J005535$-$723533 & 13.8994 & $-72.593$ & 15 & C & 0.162 & $>1.38$ & 7.2 & $529^{+206}_{-125}$ & $1.23^{+0.05}_{-0.04}$ \\
221 & J005642$-$725216 & 14.1764 & $-72.871$ & 25 & C & 0.125 & $>1.58$ & 7.8 & $282^{+41}_{-32}$ & $1.25^{+0.04}_{-0.03}$ \\
222 & J005644$-$725200 & 14.1872 & $-72.867$ & 39 & C & 0.087 & $>1.94$ & 8.0 & $279^{+24}_{-23}$ & $1.21^{+0.03}_{-0.02}$ \\
\hline
\end{tabular}

